In-context Examples Selection for Machine Translation

Large-scale generative models show an impressive ability to perform a wide range of Natural Language Processing (NLP) tasks using in-context learning, where a few examples are used to describe a task to the model. For Machine Translation (MT), these examples are typically randomly sampled from the development dataset with a similar distribution as the evaluation set. However, it is unclear how the choice of these in-context examples and their ordering impacts the output translation quality. In this work, we aim to understand the properties of good in-context examples for MT in both in-domain and out-of-domain settings. We show that the translation quality and the domain of the in-context examples matter and that 1-shot noisy unrelated example can have a catastrophic impact on output quality. While concatenating multiple random examples reduces the effect of noise, a single good prompt optimized to maximize translation quality on the development dataset can elicit learned information from the pre-trained language model. Adding similar examples based on an n-gram overlap with the test source significantly and consistently improves the translation quality of the outputs, outperforming a strong kNN-MT baseline in 2 out of 4 out-of-domain datasets.

==> backup/indomain_main.tex <==
\begin{table*}[t]
\centering
 % \setlength\tabcolsep{3.5pt}
% \scalebox{0.90}{
\begin{tabular}{lcrrrrr}
 \toprule
\bf{Selection Method}& $\bf{p+q_{max}}$  & {\bf{De-En}} &  {\bf{En-De}}& {\bf{Ru-En}}   &  {\bf{En-Ru}} & \bf{Avg.} \\ 
  \midrule
   \rowcolor{gray!10}  \multicolumn{2}{l}{\bf{\textit{ Few-shot}}} \\
    \addlinespace[0.2cm]
Random-Avg & \colorbox{paleyellow}{$16+0$} & 31.26 \small$\pm 0.26$  & 24.48 \small$\pm 0.11$  & 30.38  \small$\pm 0.65$  & 25.67  \small$\pm 0.79$ & 27.95 \\
    \addlinespace[0.2cm]
\multirow{3}{*}{Task-level} & \colorbox{pink}{$1+0$} & 32.16  & 23.35  & 30.48  & 25.04 & 27.75 \\
 \addlinespace[0.1cm]
 & \colorbox{tiffanyblue}{$4+0$} &  31.13 & 23.73  & 30.71  &27.00 & 28.14 \\
  \addlinespace[0.1cm]
  & \colorbox{paleyellow}{$16+0$} &   31.22  &23.72 & 30.89  & 27.27 & 28.28 \\

\addlinespace[0.2cm]
 \rowcolor{gray!10}  \multicolumn{2}{l}{\bf{\textit{Retrieved \incontext}}} \\
     \addlinespace[0.2cm]
\multirow{3}{*}{\bm} & \colorbox{pink}{$0+1$} & 25.82 & 19.17 & 24.54 &21.51 & 22.76\\
\addlinespace[0.1cm]
    & \colorbox{tiffanyblue}{$0+4$} & 31.02 & 24.05 &29.81 & 25.86 & 27.69 \\
    \addlinespace[0.1cm]
    & \colorbox{paleyellow}{$0+16$} & 32.16 &26.58 &  31.44 &28.54 & 29.68\\
    \addlinespace[0.1cm]
     & \colorbox{mint}{$0+17$} & 32.40 & 26.59 & 31.35 & 28.65 & 29.75\\
    \addlinespace[0.2cm]


\addlinespace[0.2cm]
 \rowcolor{gray!10}  \multicolumn{2}{l}{\bf{\textit{Retrieved Reranked \incontext}}} \\
 \addlinespace[0.2cm]
\multirow{3}{*}{R-\bm} & \colorbox{pink}{$0+1$}  & 28.19   & 20.60 & 27.26 &  21.92 & 24.49 \\
\addlinespace[0.1cm]
    & \colorbox{tiffanyblue}{$0+4$} & 31.03 & 25.32  & 30.62 &27.13 & 28.53\\
    \addlinespace[0.1cm]
    & \colorbox{paleyellow}{$0+16$} & 32.59 & 27.07 & 31.85 &28.90 & 30.10\\
    \addlinespace[0.1cm]
     & \colorbox{mint}{$0+17$} & 32.68 & 27.00 & 31.88 &28.80 & 30.09\\
    \addlinespace[0.2cm]

 \rowcolor{gray!10}  \multicolumn{2}{l}{\bf{\textit{Mixed \incontext}}} \\
 % 1-Best + \bm & \multirow{2}{*}{\colorbox{mint}{$1+16$}} & 32.92 & 26.71 & 31.64 &28.77 & 30.01 \\
 % \addlinespace[0.1cm]
1-Best + R-\bm &   \colorbox{mint}{$1+16$} & \bf{33.24} & \bf{27.09} & \bf{31.90} &  \bf{29.50} & \bf{30.43} \\
  \bottomrule
 \end{tabular}
 % }
\caption{Results on \textsc{WMT}'19 test sets.}\label{tab:main_ind_eval} 
\end{table*}



==> backup/out_of_domain_results.tex <==
\begin{table*}[t]
\centering
\scalebox{0.90}{
\begin{tabular}{llcrrrrr}
 \toprule
\bf{Method}& \bf{Corpus} & $\bf{p+q_{max}}$  & {\bf{MEDICAL}} & {\bf{LAW}} & {\bf{IT}}   &  {\bf{KORAN}}  &  {\bf{Avg.}}  \\ 
  \midrule
  \addlinespace[0.2cm]
\multirow{4}{*}{Task-level} &  Out-of-domain (Train) & \multirow{2}{*}{\colorbox{pink}{$1+0$}} & 31.23 & 32.10 & 28.70 & 14.68 & 26.68 \\
& \textsc{WMT} (Train)  &  &  30.12 & 31.10 &  26.72 & 13.19 & 25.28 \\
 \addlinespace[0.2cm]
& Out-of-domain (Train)  & \multirow{2}{*}{\colorbox{paleyellow}{$16+0$}} & 32.65 & 33.68 & 28.81 & 15.30 & 27.61 \\
&  \textsc{WMT} (Train) &  & 30.16 & 30.76 & 26.19 & 12.70 & 24.95\\
    \addlinespace[0.2cm]

      \rowcolor{gray!10}  \multicolumn{2}{l}{\bf{\textit{Retrieved Reranked \incontext}}} \\
 \multirow{3}{*}{R-\bm} &  \multirow{3}{*}{Out-of-domain (Train)}  & \colorbox{pink}{$0+1$} & 52.62 & 55.46  & 40.54 & 13.76 & 40.60\\
  % \addlinespace[0.1cm]
  %  &  & \colorbox{tiffanyblue}{$0+4$} & 54.61 & 58.89 & 45.33 & 16.11 & 43.74\\
   \addlinespace[0.1cm]
    &  & \colorbox{paleyellow}{$0+16$} & 56.43 & \bf{59.57} & 46.57  & 17.49 & 45.02 \\
    \addlinespace[0.1cm]
      &  & \colorbox{mint}{$0+17$} &  56.65 & 59.55 & 46.64 & 17.48 & 45.08 \\
  \rowcolor{gray!10}  \multicolumn{2}{l}{\bf{\textit{Mixed \incontext}}} \\
   \addlinespace[0.2cm]
   
 1-Best (I) + R-\bm &     Out-of-domain (Train)   &    \colorbox{mint}{$1+16$}  & \bf{56.76} & 59.56 & \bf{47.50} & \bf{17.55} & \bf{45.34} \\ 

  \addlinespace[0.2cm]
  \midrule
  \textsc{kNN-MT} & - & -  & 54.35 & 61.78 & 45.82 & 19.45 & 45.35\\
  \bottomrule
 \end{tabular}
 }
\caption{Results on the Multi-Domain Test Set: Prompting XGLM with the reranked prompts outperforms kNN-MT on 2 out of 4 domains.}\label{tab:main_ood_eval} 
\end{table*}

% \todo{Sweta}{Add number of examples accessed in total: https://openreview.net/pdf?id=uu1GBD9SlLe}


